Pacer: Comprehensive Network Side-Channel Mitigation in the Cloud

Network side channels (NSCs) leak secrets through packet timing and packet sizes. They are of particular concern in public IaaS Clouds, where any tenant may be able to colocate and indirectly observe a victim's traffic shape. We present Pacer, the first system that eliminates NSC leaks in public IaaS Clouds end-to-end. It builds on the principled technique of shaping guest traffic outside the guest to make the traffic shape independent of secrets by design. However, Pacer also addresses important concerns that have not been considered in prior work -- it prevents internal side-channel leaks from affecting reshaped traffic, and it respects network flow control, congestion control and loss recovery signals. Pacer is implemented as a paravirtualizing extension to the host hypervisor, requiring modest changes to the hypervisor and the guest kernel, and only optional, minimal changes to applications. We present Pacer's key abstraction of a cloaked tunnel, describe its design and implementation, prove the security of important design aspects through a formal model, and show through an experimental evaluation that Pacer imposes moderate overheads on bandwidth, client latency, and server throughput, while thwarting attacks based on state-of-the-art CNN classifiers.

==> Makefile <==
PAPER = pacer
TEX = $(wildcard *.tex)
BIB = pacer.bib
#FIGS = $(wildcard figures/*.pdf plots/*.pdf)
FIGS = $(wildcard ./*.png)
PLOTS	= mwxputlat-all-subplots	\
        padding	\
        padding-wiki	\
        videomaxrtt	\
				stat-masking-24h	\
        stat-nomasking-24h	\

.SUFFIXES: .plot .eps .fig .png .pdf

all: graphs figures $(PAPER).pdf

#plots/%.pdf: plots/%.py plots/%.csv
#	python $<

graphs: $(addprefix ./, $(addsuffix .pdf, $(PLOTS)))

figures: $(addprefix ./, $(FIGS))

$(PAPER).aux: $(TEX)
	pdflatex $(PAPER).tex

$(PAPER).bbl: $(PAPER).aux $(PAPER).bib
	bibtex $(PAPER)

$(PAPER).pdf: $(TEX) $(PAPER).bbl
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex

#$(PAPER).pdf: $(TEX) $(BIB) jpaper.cls
#	echo $(FIGS)
#	pdflatex $(PAPER)
#	bibtex $(PAPER)
#	pdflatex $(PAPER)
#	pdflatex $(PAPER)

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf

BASE ?= HEAD^
HEAD ?= HEAD

BASE_SHORT ?= $(shell git rev-parse --short ${BASE})
HEAD_SHORT ?= --

# (1) clone https://gitlab.com/git-latexdiff/git-latexdiff
# (2) cd git-latexdiff && make && make install
# (3) run 'make diff BASE=<version you want to compare against>'
diff::
	git latexdiff --main ${PAPER}.tex --latexmk  \
		${BASE_SHORT} ${HEAD_SHORT} \
		-o ${PAPER}-diff.pdf \
		--ignore-latex-errors --view	\
		--exclude-safecmd="todo,update,am,dg,pd,mz"


.PHONY: all clean

